Relational Response Fields: A General Theory of Black-Box LLM Response Consistency and Recovery

Black-box language-model reliability is commonly pursued by sampling, prompting, voting, verifying, or iteratively revising individual answers. We ask a prior question: \emph{what determines whether a collection of black-box responses is recoverable at all?} We represent responses to typed transformations of a query as a \emph{relational response field} (RRF). Edge transports encode how valid responses must change under paraphrase, scaling, decomposition, refactoring, or other task symmetries; anchors encode independently trusted evidence such as execution or a verifier. For relation operator $D$, anchor operator $A$, and at most $k$ corrupted response nodes, we identify $\gamma_k(D,A)$ as the intrinsic difficulty of black-box response recovery. It is positive exactly when every $k$-node corruption is identifiable; it gives a deterministic stability bound proportional to $1/\gamma_k$; and a matching two-point minimax lower bound shows that no estimator can improve this dependence. Thus consistency is not truth: relation-only methods are blind to null directions, including shared hallucinations. We derive sparse field-repair algorithms while separating information-theoretic identifiability from the stronger null-space conditions required by convex optimization. Controlled theorem tests and black-box mathematics/code experiments evaluate four theory-fixed consequences: consistency--truth separation, anchor phase transitions, redundancy saturation, and cross-model, cross-task prediction of repair difficulty. The results support $\gamma_k(D,A)$ as a measurable property of a response-recovery instance, rather than a score attached to one repair heuristic.

==> tables/main_replay_correlations.tex <==
\begin{tabular}{lrr}
\toprule
Model--task stratum & Replay fields & Spearman $\rho$\\
\midrule
Phi-3-mini--code & 220 & 0.397\\
Qwen-0.5B--code & 650 & 0.506\\
Phi-3-mini--mathematics & 1260 & 0.460\\
Qwen-0.5B--mathematics & 560 & 0.385\\
\midrule
Pooled & 2690 & 0.449\\
\bottomrule
\end{tabular}

